MeeQA: Natural Questions in Meeting Transcripts

We present MeeQA, a dataset for natural-language question answering over meeting transcripts. It includes real questions asked during meetings by its participants. The dataset contains 48K question-answer pairs, extracted from 422 meeting transcripts, spanning multiple domains. Questions in transcripts pose a special challenge as they are not always clear, and considerable context may be required in order to provide an answer. Further, many questions asked during meetings are left unanswered. To improve baseline model performance on this type of questions, we also propose a novel loss function, \emph{Flat Hierarchical Loss}, designed to enhance performance over questions with no answer in the text. Our experiments demonstrate the advantage of using our approach over standard QA models.

==> experiments.tex <==
\section{Experimental Setup}
\subsection{Data Representation}
We consider three different options for representing a transition between two consecutive utterances and representing the question used as an input for all the models. Figure 5 presents an example of the different representations for a sequence.

\begin{itemize}
    \item \textbf{Original:} This option serves as a baseline where the data and the questions are represented in their original format. A special token separates every two utterances, ``\&'', followed by the speaker token (as defined in  \cref{subsec:model}), and we pass the model just the question, without any previous utterances, i.e., $k=0$.
    \item \textbf{OnlySwitchSpeakers:} In this representation, we use the token representing a new utterance and the speaker token only when the speaker of the current utterance is not the same as the one of the previous one. Regarding the question representation, we consider two options:
    \begin{itemize}
        \item[$\ast$] \textbf{Original:} We pass the model just the question without previous utterances, i.e., $k=0$.
        \item[$\ast$] \textbf{PreviousUtterance:} We pass the model the question as a concatenation of one utterance before it and the question itself, i.e., $k=1$, and $U_B=u_{-1}$.
    \end{itemize}
\end{itemize}

\subsection{Evaluation Metrics}
Following SQuAD \citep{squad}, we evaluate our performance by two metrics; Exact Match (EM) and macro-average F1 score. Long sentences characterize answers in our dataset as opposed to short evidence; thus, we opt for an index-level F1-score instead of a word-level score. Recall and precision are computed by considering the overlap between predicted word indices and ground truth answers. Questions without an answer are assigned an F1 score of 1 if the model predicted ``no answer'' and 0 otherwise. We consider a question to be unanswerable if at least half of the judges tagged it as such. In SQuAD, each model prediction is compared to $n$ annotated answers for computing these metrics, and the maximum score is chosen as the question score. However, for computing human performance, each human annotation is compared to the other $n-1$ annotations. Thus, the human performance and the model results are not comparable. To moderate this bias, we compare the model results to $n$ subsets of $n-1$ annotated answers, and the final scores are calculated as the average of the maximum scores of all subsets, similar to \citet{coqa} and \citet{quaq}.

\subsection{Baseline Models}
\paragraph{Base Models} - For each of the pre-trained language models we consider BERT \citep{bert}, DeBERTa \citep{deberta}, and ALBERT \citep{albert}), we compare our hierarchal loss function to the one that was proposed in \citet{bert}. Namely, the training objective of each pre-trained language model is to maximize the sum of the log-likelihood of the correct start and end position.

\paragraph{First Utterance}
This is a naive baseline that, given a question, predicts the whole first utterance after it, i.e., $u_1$, to be the answer. We consider this baseline since most of the answers in our dataset contain the first utterance.

\subsection{Ablation Models}
We consider three additional variants of our model that aim to examine the effect of the three components in our loss in \cref{eq:hierarchical_loss}. Each ablation model trains to minimize a loss function with only two of the three components:

\noindent\textbf{No-HA-Loss} - this model trains to minimize the following loss function:
\begin{equation}
	\begin{split}
        \mathcal{L} = \frac{1}{N} ( 
        \beta \cdot \sum\limits_{i=1}^{N}\hat{y}_{HA}\cdot \mathcal{L}_{SE}(X_i)\ + \\ 
        \gamma \cdot \sum\limits_{i=1}^{N} y_{HA}\cdot \mathcal{L}_{SE}(X_i))
	\end{split}
	\end{equation}
\noindent\textbf{No-PSE-Loss} - this model trains to minimize the following loss function:
\begin{equation}
	\begin{split}
        \mathcal{L} = \frac{1}{N} (\alpha \cdot \sum\limits_{i=1}^{N}\mathcal{L}_{HA}(X_i) + \\ 
        \gamma \cdot \sum\limits_{i=1}^{N} y_{HA}\cdot \mathcal{L}_{SE}(X_i))
	\end{split}
	\end{equation}
\noindent\textbf{No-LSE-Loss} - this model trains to minimize the following loss function:
\begin{equation}
	\begin{split}
        \mathcal{L} = \frac{1}{N} (\alpha \cdot \sum\limits_{i=1}^{N}\mathcal{L}_{HA}(X_i) + \\ 
        \beta \cdot \sum\limits_{i=1}^{N}\hat{y}_{HA}\cdot \mathcal{L}_{SE}(X_i))
	\end{split}
	\end{equation}

\subsection{Implementation Details}
We use the huggingface Transformers library \citep{transformers_huggingface}\footnote{\url{https://github.com/huggingface/transformers}} to implement our models. We adopt the available pre-trained language models: BERT, DeBERTa, and ALBERT, and add on top of them the three linear classifiers as described in \cref{eq:softmax1},\cref{eq:softmax2} and \cref{eq:softmax3}, and implement the loss function as described in \cref{eq:hierarchical_loss}.

We train all models for two epochs and optimize their parameters with the ADAMW optimizer \citep{adam}. We employ a batch size of 8 and a learning rate of $3 \cdot 10^-5$. The number of utterances after the questions is $l=60$ for all experiments, and the maximum input length for all models is 512 tokens. We truncate long sequences and pad shorter ones to the maximum input length. 

For the models that use our hierarchical loss function, we tune the $\alpha$ parameter considering the values $\{0.7, 0.8\}$, the $\beta$ parameter considering the values $\{0.2, 0.3\}$, and the $\gamma$ parameter  considering the values $\{0.7, 0.8\}$. For the answer verification step, we consider the values $\{0.6, 0.7\}$ for $\tau_1$, and the values $\{0.8, 0.9\}$ for $\tau_2$. For all models, we consider the values $\{200, 250\}$ for the maximum answer length, $m$.
